Support Size Estimation: The Power of Conditioning

We consider the problem of estimating the support size of a distribution $D$. Our investigations are pursued through the lens of distribution testing and seek to understand the power of conditional sampling (denoted as COND), wherein one is allowed to query the given distribution conditioned on an arbitrary subset $S$. The primary contribution of this work is to introduce a new approach to lower bounds for the COND model that relies on using powerful tools from information theory and communication complexity. Our approach allows us to obtain surprisingly strong lower bounds for the COND model and its extensions. 1) We bridge the longstanding gap between the upper ($O(\log \log n + \frac{1}{\epsilon^2})$) and the lower bound $\Omega(\sqrt{\log \log n})$ for COND model by providing a nearly matching lower bound. Surprisingly, we show that even if we get to know the actual probabilities along with COND samples, still $\Omega(\log \log n + \frac{1}{\epsilon^2 \log (1/\epsilon)})$ queries are necessary. 2) We obtain the first non-trivial lower bound for COND equipped with an additional oracle that reveals the conditional probabilities of the samples (to the best of our knowledge, this subsumes all of the models previously studied): in particular, we demonstrate that $\Omega(\log \log \log n + \frac{1}{\epsilon^2 \log (1/\epsilon)})$ queries are necessary.

==> upperbound.tex <==
\section{Upper bound} \label{sec:upperbound}
We give an algorithm that makes $O(\log \log n + \frac{1}{\epsilon^2})$ queries to the Subset Sample oracle and   estimates the support size within multiplicative $(1+\epsilon)$-factor with high probability. We also show that for multiplicative constant approximation, only $O(\log \log n)$ queries to the Subset Query is required.
 Our results improve the previous best known upper bound of $O(\frac{\log \log n}{\epsilon^3})$\cite{} (when access to $\CO$ is given) and almost matches our lower bound.   Our upper bound holds for general case, i.e., without any assumption on the minimum probability (to be at least $\frac{\Omega(1)}{n}$) which is crucial in all the earlier works.
 Further, we use the weaker oracle for our upper bound --- Subset Query for multiplicative constant approximation and Subset  Sample for multiplicative $(1+\epsilon)$-approximation, compared to earlier stronger $\CO$  model. Thus our work substantially strengthens the previous results. 

 %Recall that in Subset Query model, given any $S \subseteq [n]$, the oracle determines if  $\sum_{i \in S} p_i = 0$ or not whereas in Subset Adversary Samples, additionally if $\sum_{i \in S} p_i > 0$ then the oracle returns an arbitrary element $i \in S$. As before, we use $\mathcal{S}$ for the support of the probability distribution. We note the following claim.
\begin{claim}
\label{clm:dquery}
Consider any $S \subseteq [n]$ and an integer $d \ge 0$. By $(d+1)$  Subset  Sample queries, it can be determined  if $|S \cap \mathcal{S}|$ is $> d$ or not and additionally  if $|S \cap \mathcal{S}| \le d$ then the set $S \cap \mathcal{S}$ can be obtained.  
\end{claim}
\begin{proof}
We first perform Subset Sample query on set $S$.   Either we get to know  $|S \cap \mathcal{S}| = 0$ in which case we are done or otherwise we get an element $e_1 \in S \cap \mathcal{S}$. Next we query the set $S\setminus \{e_1\}$. If  $|(S\setminus \{e_1\}) \cap \mathcal{S}| = 0$ then we know $|S \cap \mathcal{S}| = 1$ and obtain the set $\{e_1\} = S \cap \mathcal{S}$  (and we are done). Otherwise we get an another element $e_2 \in (S \cap \mathcal{S})\setminus \{e_1\}$. In this way, after  $d+1$ queries,  we know if $|S \cap \mathcal{S}| \le  d$ or not and if $|S \cap \mathcal{S}| \le d$ and we obtain the set $S \cap \mathcal{S}$.
\end{proof}
%Note that in Subset Adversary Samples,

%For the below upper bound, we only need an oracle that for any $S \subseteq [n]$, either can tell $\sum_{i \in S} p_i = 0$ and returns any (arbitrary) element $i \in S$ with $p_i > 0 $   otherwise. Obviously COND oracle has this property. If $x'$ is the number of elements in $S$ with positive probability, by at most $x$ oracle access, we can determine  $\min\{x,x'\}$ distinct elements in $S$ with positive probability. This can be done iteratively: first we find an element $y_1$ in $S$ with positive probability  (by oracle access on $S$) then we find an element $y_2 \in S \setminus y_1$ with positive probability (by oracle access on $S \setminus y_1$). Similarly, we can find an element $y_i \in S \setminus \{y_1,\dots,y_{i-1}\}$ with positive probability for all $i \le \min\{x,x'\}$. 
Our algorithm is inspired from the algorithm to  count distinct elements in a stream by Bar Yossef et al. \cite{}.
\begin{theorem}
\label{thm:upperbound}
\begin{enumerate}
    \item There is an algorithm that given Subset Query access to a distribution $D$ on $[n]$,  estimates the support size $s = |Supp(D)|$ to a multiplicative $f = 4\sqrt{2}$-factor with probability at least $0.55$, i.e., returns $\hat{s}$ satisfying $\frac{s}{f} \le \hat{s} \le f s$, using at most $O(\log \log n)$ queries to the oracle.
    \item There is an algorithm that given Subset Sample access to a distribution $D$ on $[n]$ and $\epsilon > 0$,  estimates the support size $s = |Supp(D)|$ to a multiplicative $(1+\epsilon)$-factor with probability at least $0.61$, i.e., returns $\hat{s}$ satisfying $(1-\epsilon) s \le \hat{s} \le (1+\epsilon) s$, using at most $O(\log \log n + \frac{1}{\epsilon^2})$ queries to the oracle.
\end{enumerate}
%There is a randomized algorithm that with high probability,  finds the support size within multiplicative $2$-factor by $O(\log \log n)$ Subset Queries and multiplicative         $(1+\epsilon)$-factor by $O(\log \log n + 1/\epsilon^2)$ Subset  Samples.
\end{theorem}
\begin{proof}
The algorithm picks a pairwise independent random hash function $h:[n] \rightarrow [n]$. Here we assume $n$ is a power of $2$ (if not then we add few elements to make $n$ equal to nearest power of $2$ and give new elements zero probability). For $t = 0,1,\dots,\log n$, let $h_t: [n] \rightarrow [2^t]$ be the projection of $h$ on its last $t$ bits. Note that $h_t$ is also a pairwise independent hash function. Also $h^{-1}_t(0) \subseteq h^{-1}_{t-1}(0)$. 


For the multiplicative $f = 4\sqrt{2}$-approximation, the algorithm does a binary search to find $t'$ such that $|h^{-1}_{t'}(0) \cap \mathcal{S}| = 0$ and $|h^{-1}_{t'-1}(0) \cap \mathcal{S}| >  0$ and then return $\frac{2^{t'}}{\sqrt{2}}$. Note that by querying the Subset Query oracle on set $h^{-1}_{t}(0)$, it can be determined if $|h^{-1}_{t}(0) \cap \mathcal{S}| >  0$ or not  (for any $t$).
  Since $|h^{-1}_{t}(0) \cap \mathcal{S}|  \le |h^{-1}_{t-1}(0) \cap \mathcal{S}|$  for all $t$, the value of $t'$ can be found after $O(\log \log n)$ queries to the Subset Query. We will prove later that, with  probability at least $0.505$, $|\mathcal{S}| \in (\frac{2^{t'}}{8}, 4 \cdot 2^{t'}]$. 

For multiplicative $(1+\epsilon)$-approximation, the algorithm finds the minimum  $t$ (say $t^*$) for which $r = |h^{-1}_t(0) \cap \mathcal{S}| \le \frac{c}{\epsilon^2}$ and    $|h^{-1}_{t-1}(0) \cap \mathcal{S}| > \frac{c}{\epsilon^2}$ (The constant $c$ is set to be 576. If $|h^{-1}_0(0) \cap \mathcal{S}| \le \frac{c}{\epsilon^2}$ then we have $t^* = 0$). The algorithm returns $r 2^{t^*}$.  We show  $t^*$ can be found by $O(1/\epsilon^2)$ queries to Subset Sample oracle, after finding $t'$.
%Now we show, after finding $t'$,   the algorithm will find $t^*$ in $(2 c/\epsilon^2)$ queries. 
To determine $t^*$, the algorithm sequentially checks which of $t',t'-1,\dots$ is $t^*$. Our algorithm  terminates if none of $t',t'-1,\dots,t' - \frac{c}{\epsilon^2}$ is $t^*$ (we will show later that with high probability, $t' \ge t^* \ge t' - \frac{c}{\epsilon^2}$). Let $T^i =  h^{-1}_{t'-i}(0) \cap \mathcal{S}$. Note that $|T^0| = 0 < c/\epsilon^2$. So if $j^*$ is the minimum $j \ge 1$ for which $|T^j| > c/\epsilon^2$ then $t^* = t'-j+1$. Thus trivially in $j^* (c/\epsilon^2 +1)$ queries (from Claim \ref{clm:dquery}), the algorithm can find $j^*$ (and hence $t^*$) (by checking if  $|T^j| >$ or $ \le  c/\epsilon^2$ for each $j \le j^*$). However, since $T^{j-1}  \subseteq T^{j}$ for all $j$, in order to determine if 
 $|T^j|$ is $>$ or $\le c/\epsilon^2$, it suffices to know if $|T^{j} \setminus T^{j-1}| > c/\epsilon^2 - |T^{j-1}|$. Note that the algorithm is also able to find the set $T^j$ for $j < j^*$. Thus the total number of queries, by Claim \ref{clm:dquery} will be $(|T^1| + 1) + (|T^2| - |T^1| +1) + \dots + (|T^{j^* - 1}) - |T^{j^* -2}| +1) + (c/\epsilon^2 - |T^{j^* - 1}| +1) = c/\epsilon^2 + j^*$.  Thus the number of Subset Sample queries to determine $t^*$ after $t'$ is at most $\frac{2c}{\epsilon^2}$ and hence total number of queries is  $O(\log \log n + \frac{1}{\epsilon^2})$.  

Now we analyse both of the above algorithms. Let $X_t = |h^{-1}_t(0) \cap \mathcal{S}|$ for $t = 0,1,\dots,\log n$. For any $j \in \mathcal{S}$, let $X_{t,j}$ be an indicator random variable for if $h_t(j) = 0$ or not. So $E[X_{t,j}] = Pr[h_t(j) = 0] = 1/2^t$ and $Var[X_{t,j}] \le E[X_{t,j}]$. Also, $E[X_t] = \sum_{j \in \mathcal{S}}X_{t,j} = |\mathcal{S}|/2^t$ and since $X_{t,j}$ are pairwise independent for any fixed $t$, we have $Var[X_t] = \sum_{j \in \mathcal{S}}Var[X_{t,j}] \le E[X_t]$. By Chebyshev's inequality, we have $\Pr[|X_t - \E[X_t]| \ge \delta \E[X_t]] \le \frac{Var[X_t]}{\delta^2 (\E[X_t])^2} \le \frac{1}{\delta^2 \E[X_t]}$.

We first show that with  probability at least $0.55$, $|\mathcal{S}| \in (\frac{2^{t'}}{8}, 4 \cdot 2^{t'}]$. Let $t_1$ be the largest value of $t$ such that $\frac{|\mathcal{S}|}{2^t} \ge 4$ and $t_2$ be the smallest value of $t$ such that $\frac{|\mathcal{S}|}{2^t} \le \frac{1}{4}$. By Markov inequality, $\Pr[X_{t_2} \ge 1] \le \E[X_{t_2}] \le \frac{1}{4}.$ Also, by Chebyshev's inequality, $\Pr[X_{t_1} =0] \le \Pr[|X_{t_1} - \E[X_{t_1}]| > 0.99 \E[X_{t_1}] ] \le \frac{1}{0.99^2 \E[X_{t_1}]} \le \frac{1}{0.99^2 \cdot  4} \le 0.26$. Therefore, with probability at least $0.76 \cdot \frac{3}{4} = 0.555$,  we have  $X_{t_2} = 0$ and $X_{t_1} > 0$ which implies  $t' > t_1$ and $t' - 1 < t_2$, i.e., $t_1 + 1 \le  t' \le t_2$. Note that $\frac{|\mathcal{S}|}{2^{t_1+1}} < 4$ and $\frac{|\mathcal{S}|}{2^{t_2 -1}} > \frac{1}{4}$. Hence, $|\mathcal{S}| \in (\frac{2^{t'}}{8}, 4 \cdot 2^{t'}]$ with probability at least $0.55$. This proves the first part of the theorem.

As shown, we have $\Pr[t' \le t_2] \ge \frac{3}{4}$. Therefore, with probability at least $\frac{3}{4}$, we have  $\E[X_{t'}] = \frac{|\mathcal{S}|}{2^{t'}} \ge \frac{|\mathcal{S}|}{2^{t_2}} > \frac{1}{8}$ and
  hence   $E[X_{t' - j}] \ge \frac{2^{j}}{8}$ for any $j \ge 1$. Therefore, conditioned on $\E[X_{t'}] \ge \frac{1}{8}$, we have $\Pr[X_{t' - \frac{c}{\epsilon^2}} \le \frac{c}{\epsilon^2}] < \Pr[|X_{t' - \frac{c}{\epsilon^2}} - \frac{2^{\frac{c}{\epsilon^2}}}{8}| > \frac{1}{2} \cdot \frac{2^{\frac{c}{\epsilon^2}}}{8}] < \frac{32}{2^{\frac{c}{\epsilon^2}}} < \frac{32}{2^c}$.
   Thus with probability at least $\frac{3}{4} \cdot \frac{32}{2^c} > 0.74$, we have $j^* \le \frac{c}{\epsilon^2}$. % Thus total queries to find $t^*$ after $t'$ is at most $c/\epsilon^2 + j^* \le 2c/\epsilon^*.$ 
 It follows from the analysis in \cite{} that the probability  $2^{t^*} X_{t^*}$ is not within the interval $[(1-\epsilon) |\mathcal{S}|, (1+\epsilon)|\mathcal{S}|$] is at most $\frac{1}{6}$. Hence, with probability at least $0.74 \cdot \frac{5}{6} = 0.61$, the algorithm is multiplicative $(1+\epsilon)$-approximation with running time $O(\log \log n + 1/\epsilon^2)$.
 For completeness, we show the proof in Appendix. 
%
\end{proof}

